Human-LLM Hybrid Text Answer Aggregation for Crowd Annotations

The quality is a crucial issue for crowd annotations. Answer aggregation is an important type of solution. The aggregated answers estimated from multiple crowd answers to the same instance are the eventually collected annotations, rather than the individual crowd answers themselves. Recently, the capability of Large Language Models (LLMs) on data annotation tasks has attracted interest from researchers. Most of the existing studies mainly focus on the average performance of individual crowd workers; several recent works studied the scenarios of aggregation on categorical labels and LLMs used as label creators. However, the scenario of aggregation on text answers and the role of LLMs as aggregators are not yet well-studied. In this paper, we investigate the capability of LLMs as aggregators in the scenario of close-ended crowd text answer aggregation. We propose a human-LLM hybrid text answer aggregation method with a Creator-Aggregator Multi-Stage (CAMS) crowdsourcing framework. We make the experiments based on public crowdsourcing datasets. The results show the effectiveness of our approach based on the collaboration of crowd workers and LLMs.

==> contents/experimental_results.tex <==
\subsection{Q1: Quality of Individual Answers by Crowd workers and LLMs}\label{sec:experiments_individual}
We investigate the individual performance of crowd creators, crowd aggregators, and LLM aggregators from the viewpoint of the quality of answers they provide or generate. Table \ref{tab:singleworkerresults} lists the results. 
First, the results in the columns of "Mean" show that both crowd aggregators and LLM aggregators can generate estimated answers with higher quality than raw crowd answers from crowd creators. 

Second, the results in the columns of "MIN", "MEAN", and "MAX" show that LLMs outperform bad and average crowd workers, but are worse than good crowd workers. Considering that model aggregators can amplify the influence of good workers when estimating true answers, a human-LLM hybrid aggregation with merged answer sets and model aggregators in the final stage has the potential to achieve better performance than aggregation results only based on crowd workers or LLMs. 

Furthermore, an observation is that the standard deviations ("STD" column) of LLM aggregators are much smaller than those of crowd creators and crowd aggregators. In such close-ended text answers, multiple LLM aggregators constructed using the same LLM with various temperature values (including relatively high values) have lower diversity than crowd creators and crowd aggregators. A potential disadvantage of low diversity is if the answer to an instance is not good, the LLM may not generate a good answer by re-generation or using diverse temperature values. High diversity in the answers is not bad for answer aggregation, because it provides a broader exploration of candidate answers and aggregation methods are proposed to estimate good workers and answers from raw answers. 

We also investigate the Inter-Annotator Agreement (IAA) among different types of workers. Because Cohen's Kappa for IAA is a statistical measure used to quantify the level of agreement between two raters who classify items into categories, while our annotations are text answers, we define a Text-Inter-Annotator Agreement (TIAA) for text answers by computing the scores between two answers to the same instance, $\kappa_{text} = \frac{1}{|\mathcal{Q}|}\sum_i \frac{1}{\mathcal{N}_{j_1,j_2}}\sum_{j_1,j_2} \mathcal{G}(a_i^{j_1},a_i^{j_2})$. $\mathcal{G}$ can be GLEU, METEOR, and Embedding Similarity. Higher TIAA means lower diversity in the answers. The results in the "TIAA" columns are based on GLEU and also show the lower diversity of LLM aggregators than crowd creators and crowd aggregators. We address this issue and candidate solution in the limitation section. 

\begin{table}[!t]
\small
\setlength\tabcolsep{3pt}
\caption{\label{tab:aggregatorperformance} Performance of different aggregators, C.A., L.A. (GPT-4 (O)), and Model Aggregator on the raw crowd answers $\mathcal{A_{C.C.}}$. }
\begin{center}
\begin{tabular}{c|cccccc}
\hline
\multirow{2}{*}{Data} & \multirow{2}{*}{C.A.} & \multicolumn{1}{c}{L.A.} & \multicolumn{3}{c}{Model Aggregator} \\
&  & (O) & SMV & SMS & RASA \\ 
\hline 
\multicolumn{6}{c}{(a) GLEU}
\\
J1 & 0.2124 & \textbf{0.2729} & 0.1930 & 0.2489 & 0.2537 \\ 
T1 & 0.1874 & 0.2184 & 0.1740 & 0.2310 & \textbf{0.2376} \\ 
T2 & 0.1817 & 0.2136 & 0.1616 & 0.2189 & \textbf{0.2340} \\ 
\hline
\multicolumn{6}{c}{(b) METEOR}
\\
J1 & 0.4156 & \textbf{0.5049} & 0.3861 & 0.4666 & 0.4745 \\  
T1 & 0.3909 & 0.4294 & 0.3786 & 0.4548 & \textbf{0.4718} \\  
T2 & 0.3840 & 0.4278 & 0.3604 & 0.4426 & \textbf{0.4653} \\ 
\hline
\multicolumn{6}{c}{(c) Embedding Similarity}
\\
J1 & 0.6857 & 0.7313 & 0.6732 & \textbf{0.7426} & 0.7414 \\ 
T1 & 0.7336 & 0.7786 & 0.7245 & 0.7935 & \textbf{0.8020} \\  
T2 & 0.7215 & 0.7651 & 0.7105 & 0.7860 & \textbf{0.7935} \\ 
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}[!t]
\scriptsize
\caption{\label{tab:aggresults_gleu} Results of text answer aggregation: GLEU; LLM aggregator (GPT-4 (O)).}
\begin{center}
\begin{tabular}{cccc|c|cc}
\hline
\multicolumn{4}{c|}{Answers} & \multicolumn{3}{c}{Model Aggregator} \\
 & $\mathcal{A}_{C.C.}$ & $\mathcal{A}_{C.A.}$ & $\mathcal{A}_{L.A.}$ & SMV & SMS & RASA \\ 
\hline
\multicolumn{7}{c}{J1}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.1930 & 0.2489 & 0.2537 \\
\cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.2260 & 0.2740 & 0.2444 \\
 & & & $\bigcirc$(O) & \textbf{0.2729} & 0.2770 & 0.2740 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.2040 & 0.2873 & 0.2708 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.2196 & 0.2846 & 0.2742 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.2494 & 0.2962 & 0.2732 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.2212 & \textbf{0.3003} & \textbf{0.2812} \\
\hline
\multicolumn{7}{c}{T1}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.1740 & 0.2310 & \textbf{0.2376} \\
\cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.1819 & 0.2074 & 0.2007 \\
 & & & $\bigcirc$(O) & \textbf{0.2184} & 0.2238 & 0.2170 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.1767 & 0.2257 & 0.2307 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.1888 & \textbf{0.2334} & 0.2218 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.2001 & 0.2249 & 0.2218 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.1871 & 0.2329 & 0.2307 \\ 
\hline
\multicolumn{7}{c}{T2}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.1616 & 0.2189 & 0.2340 \\
\cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.1769 & 0.2087 & 0.1952 \\
 & & & $\bigcirc$(O) & \textbf{0.2136} & 0.2122 & 0.2095 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.1667 & \textbf{0.2369} & 0.2341 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.1789 & 0.2293 & 0.2194 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.1953 & 0.2253 & 0.2252 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.1784 & 0.2309 & \textbf{0.2372} \\
\hline
\end{tabular}\\
\end{center}
\end{table}

\subsection{Q2: Performance of Different Aggregators}
We also compare different types of aggregators on the raw crowd answers. We use the mean results of crowd aggregators and LLM aggregators in Table \ref{tab:singleworkerresults} and add the results of the model aggregators to list them in Table \ref{tab:aggregatorperformance}. The dataset-wise model aggregator RASA that models worker reliability performs best in many cases, and performs better than instance-wise model aggregators SMV and SMS.  
LLM aggregators sometimes perform best because they not only select answers from the raw answers but also infer answers through their language understanding and reasoning ability. 

\subsection{Q3: Results on Text Answer Aggregation}
Table \ref{tab:aggresults_gleu} shows the results of text answer aggregation on the evaluation metric GLEU. $\mathcal{A}_{L.A.}$ with (O) uses GPT-4. 
To facilitate the discussions, the results are organized into four groups. Group \Rmnum{1} represents the existing work with only crowd creators and the single-stage framework; Group \Rmnum{2} is the performance of our CAMS framework with only crowd aggregators or LLM aggregators; Group \Rmnum{3} and Group \Rmnum{4} are answer aggregations with our CAMS framework with more than two answer resources; Group \Rmnum{4} includes the human-LLM hybrid combinations with LLM aggregators. \textit{Groups \Rmnum{2}, \Rmnum{3} and \Rmnum{4} are our proposals}. 
We address the major observations as follows. 

First, comparing the results among three columns, SMV performs worst in all three model aggregators. It shows that utilizing a strong model aggregator rather than a majority-based na\"ive aggregator is important for answer aggregation. Although the L.A.-only version of our approach performs best in all three datasets when using SMV, the performance is always lower than those using SMS and RASA. The following discussions will only focus on the results based on SMS and RASA. 

\begin{table}[!t]
\scriptsize
\caption{\label{tab:aggresults_meteor} Results of text answer aggregation: METEOR; LLM aggregator (GPT-4 (O)).} 
\begin{center}
\begin{tabular}{cccc|c|cc}
\hline
\multicolumn{4}{c|}{Answers} & \multicolumn{3}{c}{Model Aggregator} \\
 & $\mathcal{A}_{C.C.}$ & $\mathcal{A}_{C.A.}$ & $\mathcal{A}_{L.A.}$ & SMV & SMS & RASA \\ 
\hline
\multicolumn{7}{c}{J1}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.3861 & 0.4666 & 0.4745 \\ \cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.4397 & 0.4912 & 0.4524 \\
 & & & $\bigcirc$(O) & \textbf{0.5049} & 0.5110 & 0.5070 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.4040 & 0.5092 & 0.4946 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.4258 & 0.5166 & 0.5076 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.4723 & \textbf{0.5248} & 0.5064 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.4293 & 0.5240 & \textbf{0.5147} \\
\hline
\multicolumn{7}{c}{T1}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.3786 & 0.4548 & \textbf{0.4718} \\ \cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.3927 & 0.4330 & 0.4272 \\
 & & & $\bigcirc$(O) & \textbf{0.4294} & 0.4351 & 0.4275 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.3833 & 0.4528 & 0.4564 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.3955 & 0.4538 & 0.4378 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.4110 & 0.4406 & 0.4366 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.3948 & \textbf{0.4609} & 0.4495 \\ 
\hline
\multicolumn{7}{c}{T2}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.3604 & 0.4426 & \textbf{0.4653} \\ \cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.3746 & 0.4238 & 0.4083 \\
 & & & $\bigcirc$(O) & \textbf{0.4278} & 0.4330 & 0.4287 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.3651 & 0.4507 & 0.4551 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.3829 & 0.4523 & 0.4402 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.4012 & 0.4423 & 0.4482 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.3808 & \textbf{0.4606} & 0.4626 \\
\hline
\end{tabular}\\
\end{center}
\end{table}

\begin{table}[t!]
\scriptsize
\caption{\label{tab:aggresults_embedding} Results of text answer aggregation: Embedding Similarity; LLM aggregator (GPT-4 (O)).}
\begin{center}
\begin{tabular}{cccc|c|cc}
\hline
\multicolumn{4}{c|}{Answers} & \multicolumn{3}{c}{Model Aggregator} \\
 & $\mathcal{A}_{C.C.}$ & $\mathcal{A}_{C.A.}$ & $\mathcal{A}_{L.A.}$ & SMV & SMS & RASA \\ 
\hline
\multicolumn{7}{c}{J1}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.6732 & 0.7426 & 0.7414 \\
\cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.6983 & 0.7360 & 0.7188 \\
 & & & $\bigcirc$(O) & \textbf{0.7313} & 0.7332 & 0.7317 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.6815 & \textbf{0.7516} & \textbf{0.7459} \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.6926 & 0.7427 & 0.7356 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.7148 & 0.7413 & 0.7336 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.6940 & 0.7484 & 0.7410 \\
\hline
\multicolumn{7}{c}{T1}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.7245 & 0.7935 & \textbf{0.8020} \\
\cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} & & $\bigcirc$ & & 0.7430 & 0.7851 & 0.7758 \\
 & & & $\bigcirc$(O) & \textbf{0.7786} & 0.7807 & 0.7762 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.7306 & 0.7965 & 0.7976 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.7425 & 0.7894 & 0.7793 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.7608 & 0.7854 & 0.7807 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.7426 & \textbf{0.7993} & 0.7890 \\
\hline
\multicolumn{7}{c}{T2}
\\
\multirow{1}{*}{\Rmnum{1}} & $\bigcirc$ & & & 0.7105 & 0.7860 & \textbf{0.7935} \\ \cdashline{1-7}
\multirow{2}{*}{\Rmnum{2}} &  & $\bigcirc$ & & 0.7282 & 0.7681 & 0.7468 \\
 & & & $\bigcirc$(O) & \textbf{0.7651} & 0.7725 & 0.7673 \\
\cdashline{1-7}
\multirow{1}{*}{\Rmnum{3}} & $\bigcirc$ & $\bigcirc$ & & 0.7164 & \textbf{0.7885} & 0.7822 \\
\cdashline{1-7}
\multirow{3}{*}{\Rmnum{4}} & $\bigcirc$ & & $\bigcirc$(O) & 0.7287 & 0.7856 & 0.7744 \\
 & & $\bigcirc$ & $\bigcirc$(O) & 0.7467 & 0.7712 & 0.7728 \\
 & $\bigcirc$ & $\bigcirc$ & $\bigcirc$(O) & 0.7286 & 0.7851 & 0.7824 \\
\hline
\end{tabular}\\
\end{center}
\end{table}

Second, comparing the SMS (RASA) results between the L.A.-only version in Group \Rmnum{2} and Group \Rmnum{4}, the versions in Group \Rmnum{4} that utilize human-LLM hybrid aggregation outperform the version in Group \Rmnum{2} that only utilizes the answers of the LLM aggregators in most of the cases. In addition, the versions in Group \Rmnum{4} also always outperform the results of LLM aggregators without model aggregators. They show that, although LLM aggregators perform better than the average of crowd workers in Table \ref{tab:singleworkerresults}, the answers provided by crowd workers contain valuable information for model aggregators to generate good answers. One purpose of answer aggregation methods is to estimate good workers and good answers from the raw crowd answers (looking for the needle in a haystack). Following the observation in Table \ref{tab:singleworkerresults} that there are still good crowd workers (creators and aggregators) who perform better than LLMs (aggregators), a strong model aggregator can target such good workers and answers. In contrast to replacing crowd workers by only using LLMs, human-LLM hybrid solutions potentially have advantages. 

Third, Table \ref{tab:aggresults_meteor} and \ref{tab:aggresults_embedding} list the results on the evaluation metrics METEOR and Embedding Similarity. They reach similar observations with the evaluation metric GLEU.  
 
Fourth, regarding the performance of different components (ablations) of the proposed method within the CAMS framework, (1) the results of columns C.A. or L.A. in Table \ref{tab:aggregatorperformance} represent components that include only crowd aggregators or LLM aggregators, without the use of model aggregators; (2) Group \Rmnum{1} represents components with only crowd creators and the single-stage framework. Comparing these results with those of Groups \Rmnum{2}, \Rmnum{3} and Group \Rmnum{4} in Tables \ref{tab:aggresults_gleu}, \ref{tab:aggresults_meteor} and \ref{tab:aggresults_embedding} illustrates the effectiveness of our human-LLM hybrid aggregation approach and CAMS framework. 

\begin{figure*}[!t]
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/GLEU_Diff_Num_LLMAgg_J1_ChatGPT.pdf}
\\(a) J1
\end{minipage}
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/GLEU_Diff_Num_LLMAgg_T1_ChatGPT.pdf}
\\(b) T1
\end{minipage}
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/GLEU_Diff_Num_LLMAgg_T2_ChatGPT.pdf}
\\(c) T2
\end{minipage}
\caption{GLEU Results by different number of L.A. (GPT-4 (O)) based on SMS and RASA. }
\label{fig:diff_num_llmagg_gleu_chatgpt} 
\end{figure*}


\begin{figure*}[!t]
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/METEOR_Diff_Num_LLMAgg_J1_ChatGPT.pdf}
\\(a) J1
\end{minipage}
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/METEOR_Diff_Num_LLMAgg_T1_ChatGPT.pdf}
\\(b) T1
\end{minipage}
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/METEOR_Diff_Num_LLMAgg_T2_ChatGPT.pdf}
\\(c) T2
\end{minipage}
\caption{METEOR Results by different number of L.A. (GPT-4 (O)) based on SMS and RASA. }
\label{fig:diff_num_llmagg_meteor_chatgpt} 
\end{figure*}

\begin{figure*}[!t]
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/EmbedSim_Diff_Num_LLMAgg_J1_ChatGPT.pdf}
\\(a) J1
\end{minipage}
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/EmbedSim_Diff_Num_LLMAgg_T1_ChatGPT.pdf}
\\(b) T1
\end{minipage}
\begin{minipage}{0.315\textwidth}
\centering
\includegraphics[height=3.5cm]{Figures/EmbedSim_Diff_Num_LLMAgg_T2_ChatGPT.pdf}
\\(c) T2
\end{minipage}
\caption{Embedding Similarity Results by different number of L.A. (GPT-4 (O)) based on SMS and RASA. }
\label{fig:diff_num_llmagg_embedsim_chatgpt} 
\end{figure*}

Fifth, in the main results, we utilize the same number of LLM aggregators with crowd aggregators, we thus also investigate the influences of different numbers of LLM aggregators on the performance. Figures \ref{fig:diff_num_llmagg_gleu_chatgpt}, \ref{fig:diff_num_llmagg_meteor_chatgpt} and \ref{fig:diff_num_llmagg_embedsim_chatgpt} show the results on the evaluation metrics GLEU, METEOR and Embedding Similarity by GPT-4 LLM aggregators based on model aggregators SMS and RASA. The results by Gemini LLM aggregators are in the Appendix. No consistent patterns were observed across different datasets; sometimes, more LLM aggregators are better; sometimes, fewer LLM aggregators are better; it depends on the datasets; we cannot know which case it is in practical crowd annotations. In all cases of the J1 dataset and some cases of the T1 and T2 datasets, the results of only using one LLM aggregator are bad; using multiple LLM aggregators is recommended to avoid risk.  

Finally, the approach we propose in this work has several versions (six combinations of worker and answer resources in Groups \Rmnum{2}, \Rmnum{3}, and \Rmnum{4}). The best version depends on the specific application. If there is no prior knowledge of the target task or dataset, we recommend using all workers and answers (i.e., crowd creators, crowd aggregators, and LLM aggregators) together with a reliable model aggregator (e.g., SMS or RASA). 


==> contents/experimental_settings.tex <==
\subsection{Datasets}
To investigate our study, we need datasets that contain multiple crowd text answers for each instance as well as the golden answers. We thus utilize the real datasets J1, T1, and T2 in CrowdWSA \cite{textaggregationdataset} which involve the translated sentences of the target language by multiple crowd workers for the sentences of the source language as well as the golden translations. Table \ref{tab:dataset_statistics} lists the statistics of the three datasets. 
The crowd workers in these datasets are regarded as the crowd creators (C.C.) in our CAMS framework. Each crowd creator provides answers for a subset of all instances. 

\subsection{Experimental Settings}
\subsubsection{Crowd Aggregators}
For crowd aggregators (C.A.), we utilize a commercial crowdsourcing platform Lancers\footnote{https://www.lancers.co.jp/} to collect the estimated answers. Each instance is assigned to five crowd aggregators. Each crowd aggregator provides estimated answers for a subset of all instances. The following instructions and task descriptions are shown to the crowd aggregators when deploying the micro crowdsourcing tasks: 

\noindent
{\quoting[leftmargin=0.25cm,rightmargin=0cm]
Instructions: \textit{The data is collected for use in academic research. The collected data will be used for research on natural language processing and machine learning. The workers' nicknames will not be disclosed to any third party other than the person requesting this task. }
\endquoting}

\noindent
{\quoting[leftmargin=0.25cm,rightmargin=0cm]
Descriptions: \textit{The ten English short sentences below were written by ten non-native English speakers who translated the same one Japanese short sentence from Japanese. Read each of the English short sentences below, infer the meaning of the original Japanese text, and based on your understanding, create what you consider to be one appropriate short sentence each in Japanese and English. }
\endquoting}

The original text instructions and task descriptions used at Lancers are in Japanese. Table \ref{tab:dataset_statistics} lists the statistics of the answers $\mathcal{A_{C.A.}}$ by crowd aggregators $\mathcal{W_{C.A.}}$ collected by this work. 

\subsubsection{LLM Aggregators}
For LLM aggregators (L.A.), we utilize GPT-4\footnote{The version is gpt-4-0125-preview.} and Gemini\footnote{The version is gemini-1.5-pro-latest in May 9-14th 2024.}. L.A.(O) uses GPT-4 and L.A.(G) uses Gemini. Because Gemini results are almost always worse than GPT-4 results, we only put GPT-4 results in the main manuscript and put Gemini results in the Appendix Section. We utilize different temperature values to construct multiple LLM aggregators. The main results are based on five LLM aggregators with temperatures [0,0.25,0.5,0.75,1], with one trial conducted for each temperature. Each LLM aggregator provides answers for all instances. The following prompt is presented to the LLMs: 

\noindent
{\quoting[leftmargin=0.25cm,rightmargin=0cm]
Prompt: \textit{The following ten short English sentences were written by ten non-native English speakers who translated the same Japanese short text from Japanese to English. Please read each English sentence and infer the meaning of the original Japanese text, and based on your understanding, provide the appropriate Japanese original text and its English translation. Only output the text without showing "Japanese original text" and "English translation". \textbackslash n\textbackslash n
<1. sentence 1>\textbackslash n<2. sentence 2>\textbackslash n......<10. sentence 10>\textbackslash n.
Output format separated by " and <tab>: "Japanese original text. " <tab> "its English translation. 
 " \textbackslash n\textbackslash n} 
\endquoting}

Regarding the budget cost associated with crowd aggregators and LLM aggregators, LLMs are generally cheaper than crowd workers for annotating instances. For example, \citet{CrowdChatgptTextAnnotation} reported that ChatGPT is about twenty times cheaper than MTurk in their experiments. 
In our experiments, LLM aggregators cost less than 0.01 dollars per instance, while crowd aggregators cost around 0.36 dollars per instance, indicating a cost difference of more than thirtyfold. 

\subsubsection{Model Aggregators}
For the model aggregators, following CrowdWSA, we use the answer aggregation approaches SMV, SMS, and RASA, and utilize universal sentence encoder\footnote{https://tfhub.dev/google/universal-sentence-encoder/4. This version is newer than the one used in the public implementation of CrowdWSA, thus the results of model aggregators on the answers of only crowd creators are different from those reported in CrowdWSA. }\cite{USE} as the text encoder. 

\subsubsection{Evaluation Metrics}
We also use three evaluation metrics to verify the proposal. Two of them are GLEU\footnote{We use NLTK package: nltk.translate.gleu\_score} and METEOR\footnote{We use NLTK package: nltk.translate.meteor\_score}. We compute the average scores between estimated answers and true answers.  
The other one is the average cosine similarity between the encoder embeddings of the estimated answers and the true answers. We utilize the original target sentences in the Japanese-English parallel corpus used by CrowdWSA as the ground truth. 


==> contents/hybrid_aggregation.tex <==
\begin{table}[t!]
\small
\caption{\label{tab:dataset_statistics} Statistics of the datasets, $|\cdot|$ is the size of the sets. The answers $\mathcal{A_{C.C.}}$ by crowd creators $\mathcal{W_{C.C.}}$ is from CrowdWSA; the answers $\mathcal{A_{C.A.}}$ by crowd aggregators $\mathcal{W_{C.A.}}$ are collected by this work. }
\begin{center}
\begin{tabular}{c|ccccc}
\hline
Data & $|\mathcal{Q}|$ & $|\mathcal{W_{C.C.}}|$ &  $|\mathcal{A_{C.C.}}|$ & $|\mathcal{W_{C.A.}}|$ &  $|\mathcal{A_{C.A.}}|$ \\ \hline
J1 & 250 & 70 & 2,490 & 106 & 1250 \\ 
T1 & 100 & 42 & 1,000 & 69 & 500 \\ 
T2 & 100 & 43 & 1,000 & 71 & 500 \\  
\hline
\end{tabular}
\end{center}
\end{table}

Most of the existing work on crowdsourced annotation is based on the single-stage framework, i.e., all crowd answers are collected from crowd creators at once and the model aggregator estimates the true answers on these raw crowd answers directly. 
Figure \ref{fig:singlestageframework} shows an example of a single-stage framework for crowdsourced text answer annotation. Single-stage frameworks are limited for the requesters to flexibly set diverse additional mechanisms for improving the data quality. Multi-stage frameworks are candidate solutions to improve flexibility and quality. 

Because the crowd answers in this study are text, it is intuitive to ask LLMs to read the multiple crowd text answers to a given instance, and generate the estimated text answer. LLMs can be used as LLM aggregators. 
Similarly, crowd workers can be asked to provide the estimated answer by reading the raw crowd answers of an instance, and be used as crowd aggregators. We regard the Crowd Creator (C.C.), Crowd Aggregator (C.A.), and LLM Aggregator (L.A.) as three different types of workers. 
To distinguish these three resources of workers and answers, we define crowd creator workers and their answers as $\mathcal{W}_{C.C.}$ and $\mathcal{A}_{C.C.}$, crowd aggregator workers and their answers as $\mathcal{W}_{C.A.}$ and $\mathcal{A}_{C.A.}$, and LLM aggregator workers and their answers as $\mathcal{W}_{L.A.}$ and $\mathcal{A}_{L.A.}$.
Note that crowd creators $\mathcal{W}_{C.C.}$ and crowd aggregators $\mathcal{W}_{C.A.}$ are allowed to have overlaps; they are not necessary to be the same or completely different. This is a tractable setting for requesters in practice, because $\mathcal{A}_{C.C.}$ and $\mathcal{A}_{C.A.}$ are collected in separate stages. 

To effectively leverage these three resources of workers and answers in one crowdsourcing framework, we propose a Creator-Aggregator Multi-Stage (CAMS) framework. Figure \ref{fig:multistageframework} shows the proposed CAMS framework. In the first stage, crowd creators provide the raw crowd answers. In the next stage, we ask crowd aggregators and/or LLM aggregators to aggregate the raw crowd answers into estimated answers in their own words. In the final stage, we utilize the model aggregators on the combinations of three resources of workers and answers to generate the estimated true answers. 

There are different versions of our approach. We can combine two or three resources of workers and answers to create the merged sets, which are then used as input for the model aggregator to estimate the true answers. We provide an example based on a version that utilizes all three resources of workers and answers. Given the instance set $\mathcal{Q}$, we can construct the worker set $\mathcal{W}$ by merging three worker sets with $\mathcal{W}$ = $\mathcal{W}_{C.C.}$+$\mathcal{W}_{C.A.}$+$\mathcal{W}_{L.A.}$, and the answer set $\mathcal{A}$ by merging three answer sets with $\mathcal{A}$ = $\mathcal{A}_{C.C.}$+$\mathcal{A}_{C.A.}$+$\mathcal{A}_{L.A.}$. We use the symbol `+' rather than the symbol `$\cup$' for $\mathcal{W}$ and $\mathcal{A}$. Because the answer creation and answer aggregation are different tasks, if the same crowd worker provides answers as both crowd creator and crowd aggregator, he/she may have different behaviors and reliabilities in these two roles. We thus treat such a worker as different workers when merging the worker and answer resources. 
We can then utilize the model aggregators on these $\mathcal{Q}$, $\mathcal{W}$, and $\mathcal{A}$ to estimate the true answers, i.e., $\hat{\mathcal{Z}} = \textnormal{Agg}(\mathcal{Q}, \mathcal{W}, \mathcal{A})$ where $\textnormal{Agg}$ is one of SMV, SMS or RASA. 

\begin{table*}[t!]
\small
\setlength\tabcolsep{1.5pt}
\caption{\label{tab:singleworkerresults} Quality of individual answers by Crowd Creators (C.C.), Crowd Aggregators (C.A.) and LLM Aggregators (L.A., GPT-4 (O)) on GLEU, METEOR, and embedding similarity. }
\begin{center}
(a) GLEU\\
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{3}{*}{Data} & \multicolumn{3}{c|}{MIN} & \multicolumn{3}{c|}{MEAN} & \multicolumn{3}{c|}{MAX} & \multicolumn{3}{c|}{STD} & \multicolumn{3}{c}{TIAA} \\ 
 & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) \\ 
\hline
J1 & 0.0724 & 0.0000 & \textbf{0.2706} & 0.1868 & 0.2124 & \textbf{0.2729} & 0.5948 & \textbf{1.0000} & 0.2756 & 0.0915 & 0.1399 & 0.0018 & 0.1798 & 0.2746 & 0.7438 \\
T1 & 0.0669 & 0.0217 & \textbf{0.2144} & 0.1764 & 0.1874 & \textbf{0.2184} & 0.5534 & \textbf{0.7895} & 0.2283 & 0.0818 & 0.1297 & 0.0051 & 0.2533 & 0.3473 & 0.7809 \\
T2 & 0.0503 & 0.0000 & \textbf{0.2025} & 0.1716 & 0.1817 & \textbf{0.2136} & 0.4540 & \textbf{0.6842} & 0.2244 & 0.0838 & 0.1190 & 0.0083 & 0.2377 & 0.3371 & 0.7589 \\
\hline
\end{tabular}
\vspace{0.1cm}\\
(b) METEOR\\
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Data} & \multicolumn{3}{c|}{MIN} & \multicolumn{3}{c|}{MEAN} & \multicolumn{3}{c|}{MAX} & \multicolumn{3}{c|}{STD} & \multicolumn{3}{c}{TIAA}\\ 
 & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) \\ 
\hline
J1 & 0.2041 & 0.0490 & \textbf{0.4987} & 0.3762 & 0.4156 & \textbf{0.5049} & 0.7464 & \textbf{0.9985} & 0.5103 & 0.1037 & 0.1569 & 0.0039 & 0.3791 & 0.4910 & 0.8683 \\
T1 & 0.1781 & 0.0394 & \textbf{0.4247} & 0.3771 & 0.3909 & \textbf{0.4294} & 0.7163 & \textbf{0.9170} & 0.4392 & 0.0987 & 0.1666 & 0.0051 & 0.4763 & 0.5670 & 0.8918 \\
T2 & 0.1523 & 0.0476 & \textbf{0.4102} & 0.3630 & 0.3840 & \textbf{0.4278} & 0.6473 & \textbf{0.8288} & 0.4407 & 0.1010 & 0.1619 & 0.0103 & 0.4402 & 0.5492 & 0.8696 \\
\hline
\end{tabular}
\vspace{0.1cm}\\
(c) Embedding Similarity\\
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Data} & \multicolumn{3}{c|}{MIN} & \multicolumn{3}{c|}{MEAN} & \multicolumn{3}{c|}{MAX} & \multicolumn{3}{c|}{STD} & \multicolumn{3}{c}{TIAA} \\ 
 & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) & C.C. & C.A. & L.A.(O) \\ 
\hline
J1 & 0.4233 & 0.2243 & \textbf{0.7216} & 0.6620 & 0.6857 & \textbf{0.7313} & 0.8795 & \textbf{1.0000} & 0.7379 & 0.0687 & 0.1135 & 0.0053 & 0.6583 & 0.7286 & 0.9322 \\
T1 & 0.5827 & 0.1282 & \textbf{0.7758} & 0.7260 & 0.7336 & \textbf{0.7786} & 0.9043 & \textbf{1.0000} & 0.7824 & 0.0687 & 0.1511 & 0.0029 & 0.7252 & 0.7850 & 0.9532 \\
T2 & 0.4726 & 0.2700 & \textbf{0.7602} & 0.7077 & 0.7215 & \textbf{0.7651} & 0.8958 & \textbf{1.0000} & 0.7679 & 0.0861 & 0.1250 & 0.0031 & 0.7060 & 0.7752 & 0.9343 \\
\hline
\end{tabular}
\end{center}
\end{table*}


==> contents/modal_aggregators.tex <==
\subsection{Model Aggregators}
We briefly introduce several aggregation approaches from existing works as the model aggregators in this work. These approaches utilize an encoder $e(\cdot)$ to convert the text into embeddings. The embedding of an answer $a_i^j$ is defined as $e_i^j$. 

\noindent
\textbf{Sequence Majority Voting (SMV): } 
It is adapted from majority voting which is one of the most typical answer aggregation approaches. For each instance, it estimates the embeddings of the true answers by $\hat{e}_i = mean(e(\mathcal{L}_i))$, and selects the worker answer \[\hat{z}_i = \arg\max_{a_i^j} sim(e(a_i^j),\hat{e}_i).\]

\noindent
\textbf{Sequence Maximum Similarity (SMS) \cite{ModelEnsembleSummary}: } For each instance, it selects the worker answer which has the largest sum of similarity with other answers to this question. It can be regarded as creating a kernel density estimator and selecting the maximum density answer. The kernel function uses the cosine similarity. The formulation is  
\[\hat{z}_i = \arg\max_{a_i^{j_1}}\sum_{j_1\neq j_2} sim(e(a_i^{j_1}),e(a_i^{j_2})).\] 


%\subsection{Reliability Aware Sequence Aggregation}
\noindent
\textbf{Reliability Aware Sequence Aggregation (RASA) \cite{textaggregationdataset}: } 
It models the worker reliability $\theta$ to strengthen the influences of answers provided by the workers with higher estimated reliability. 
%Many existing works of the answer aggregation (not only text answers, but also other types of answers such as categorical answers) strengthen the influences of answers provided by the workers with higher estimated reliability. 
It first estimates the embeddings of the true answers considering worker reliability. It  iteratively estimates $\theta$ and $\hat{e}_i$ until convergence, \[\theta_j = \frac{{\chi}^2_{(\alpha/2,|\mathcal{A}^j|)}}{\sum(e(a_i^j)-\hat{e}_i)^2}, \hat{e}_i = \frac{\sum \theta_ke(a_i^j) }{\sum \theta_j},\]
%\[\beta_k = \frac{{\chi}^2_{(\alpha/2,|\mathcal{A}^j|)}}{\sum(e(a_i^j)-\hat{e}_i)^2},\ \ \ \hat{e}_i = \frac{\sum \beta_ke(a_i^j) }{\sum \beta_j},\]
where ${\chi}^2$ is the chi-squared distribution and the significance level $\alpha$ is set as 0.05 empirically. $\hat{e}_i$ can be initialized by using the \textsc{SMV}. 
After that, it selects a worker answer that is most similar to the embeddings of the estimated true answer. % for each instance

%following the answer aggregation approaches provided by CrowdWSA
\noindent
\textbf{Experimental settings: } For these model aggregators, following CrowdWSA, we use the answer aggregation approaches SMV, SMS, and RASA, and utilize universal sentence encoder\footnote{https://tfhub.dev/google/universal-sentence-encoder/4. This version is newer than the one used in the implementation in CrowdWSA, thus the results of model aggregators on the answers of only crowd creators are different from those reported in CrowdWSA. }\cite{USE} as the encoder. 


\iffalse
When we obtain multiple answers for a given question, we need to aggregate them into one answer which can be used as the golden data in the collected dataset.
There are at least two alternatives of answer aggregation approaches for the case of word sequence, i.e., extractive and abstractive answer aggregation. Extractive aggregation methods extract the potential optimal one from multiple worker answers; abstractive aggregation methods generate a new answer by analyzing and understanding all of the worker answers. In the research area of crowdsourcing, most of the existing work of answer aggregation focus on categorical or numerical labels \cite{LabelAggregationSurvey}. They estimate a pre-defined category or value and thus are extractive approaches. The abstractive approach is a special alternative for sequence labels. In this short paper, we focus on the baselines based on extractive answer aggregation. 

%\ffuku{Abstractive aggregation methods generate a new answer by analyzing and understanding all of the worker answers.}

The notations are as follows. We define question set $\mathcal{Q}=\{q_i\}_i$, worker set $\mathcal{W}=\{w_k\}_k$, answer set $\mathcal{A}=\{a_i^k\}_{i,k}$, true answer set $\mathcal{Z}=\{z_i\}_i$ and estimated true answer set $\hat{\mathcal{Z}}=\{\hat{z}_i\}_i$. The answer set of a question is $\mathcal{L}_i$; the answer set of a worker is $\mathcal{V}_k$. The encoder is $e(\cdot)$. We use cosine similarity for $sim$ computation. 


%\subsection{Sequence Majority Voting}
\noindent
\textbf{Sequence Majority Voting (SMV): } 
Majority voting is one of the most typical answer aggregation approaches. For the specific data type of word sequences, we adapt it into a Sequence Majority Voting (SMV) approach. For each question, it first estimates the embeddings of the true answers by $\hat{e}_i = mean(e(\mathcal{L}_i))$; after that it extracts the worker answer $\hat{z}_i = \arg\max_{a_i^k} sim(e(a_i^k),\hat{e}_i)$ as the true answer.

%\subsection{Sequence Maximum Similarity}
\noindent
\textbf{Sequence Maximum Similarity (SMS): } 
We adapt the method in \citet{ModelEnsembleSummary}, which is proposed as a post-ensemble method for multiple summarization generation models. For each question, it extracts the worker answer which has largest sum of similarity with other answers of this question. It can be regarded as creating a kernel density estimator and extract the maximum density answer. The kernel function uses the cosine similarity. This Sequence Maximum Similarity (\textsc{SMS}) method can be formulated as follows, 
$\hat{z}_i = \arg\max_{a_i^{k_1}}\sum_{k_1\neq k_2} sim(e(a_i^{k_1}),e(a_i^{k_2}))$. 


%\subsection{Reliability Aware Sequence Aggregation}
\noindent
\textbf{Reliability Aware Sequence Aggregation (RASA): } 
Both \textsc{SMV} and \textsc{SMS} do not consider the worker reliability. In crowdsourcing, worker reliability is diverse and is a useful information for estimating true answers. Existing work in the categorical answer aggregation strengthen the influences of answers provided by the workers with higher reliability. 
Therefore, we also propose an approach which models the worker reliability, named as Reliability Aware Sequence Aggregation (RASA). 

% \begin{algorithm}[t]
% \LinesNumbered
% \KwIn{Questions $\mathcal{Q}$; Workers $\mathcal{W}$; Answers $\mathcal{A}$}
% \KwOut{Estimated true answers $\hat{\mathcal{Z}}$;}
% $\mathcal{E}=\textsc{Encoder}(\mathcal{A})$\;
% $\hat{\mathcal{E}}=\textsc{Estimation}(\mathcal{Q},\mathcal{W},\mathcal{E})$\;
% $\hat{\mathcal{Z}} = \textsc{Extraction}(\mathcal{Q},\mathcal{A},\mathcal{E},\hat{\mathcal{E}})$\;
% \KwRet{$\mathcal{Z}$}
% \caption{\textsc{RASA}\label{alg:ewsa}}
% \end{algorithm}
% %Reliability Aware Sequence Aggregation

%Algorithm \ref{alg:ewsa} describes the RASA approach. 
The RASA approach is as follows.
(1). \textsc{Encoder}: it encodes the worker answers into embeddings; (2). \textsc{Estimation}: it estimates the embeddings of the true answers considering worker reliability; (3). \textsc{Extraction}: for each question, it extracts a worker answer which is most similar with the embeddings of the estimated true answer.
% it first; after that; finally

%\ffuku{"the estimated true answer" means "the estimated answer with reliability"?}

For estimating the embeddings of the true answers, we adapt the CATD approach \cite{CATD} which is proposed for aggregating multiple numerical ratings. We extend it into our sequence case by adapting it to the sequence embeddings. We define the worker reliability as $\beta$. %The optimization problem is defined as follows. 
%\[\min_{\beta} \sum_k \beta_k^2\frac{1}{|\mathcal{V}_k|}\sum_{a_i^k\in \mathcal{V}_k}(e(a_i^k)-\hat{e}_i)^2,\] \[s.t., \sum_k \beta_k = 1, \beta_k \ge 0.\]
%It is optimized by iteratively updating $\beta_k$ and $\hat{e}_i$, 
The method iteratively estimates $\beta_k$ and $\hat{e}_i$ until convergence,
\[\beta_k = \frac{{\chi}^2_{(\alpha/2,|\mathcal{V}_k|)}}{\sum(e(a_i^k)-\hat{e}_i)^2},\ \ \ \hat{e}_i = \frac{\sum \beta_ke(a_i^k) }{\sum \beta_k},\]
where ${\chi}^2$ is the chi-squared distribution and the significance level $\alpha$ is set as 0.05 empirically. We initialize $\hat{e}_i$ by using the \textsc{SMV} approach.
\fi

==> contents/problem_setting.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=11cm]{Figures/single-stage framework.jpg}
\caption{Existing Single-Stage framework for crowdsourced text answer aggregation.}
\label{fig:singlestageframework} 
\end{figure*}

\begin{figure*}[!t]
\centering
\includegraphics[width=16cm]{Figures/multi-stage framework.jpg}
\caption{Our Creator-Aggregator Multi-Stage (CAMS) framework for crowdsourced text answer aggregation. }
\label{fig:multistageframework} 
\end{figure*}

\subsection{Problem Setting of Answer Aggregation}
We formulate the general problem setting of crowd text answer aggregation for quality control in close-ended text answer annotations. 
We define the instance set $\mathcal{Q}=\{q_i\}_i$, worker set $\mathcal{W}=\{w_j\}_j$, answer set $\mathcal{A}=\{a_i^j\}_{i,j}$, where $a_i^j$ represents the answer to question $q_i$ by worker $w_j$, true answer set $\mathcal{Z}=\{z_i\}_i$ and estimated answer set $\hat{\mathcal{Z}}=\{\hat{z}_i\}_i$. 
The answer set of an instance $q_i$ is $\mathcal{A}_i$; the answer set of a worker $w_j$ is $\mathcal{A}^j$. Because the number of instances can be large, a worker is not necessary to annotate all instances. 

In the setting of the crowd answer aggregation, ground truths cannot be used by model aggregators because the purpose of data annotation tasks is collecting and estimating the ground truth.  
Therefore, abstractive aggregation methods, such as abstractive text summarization, which require ground truth for training, are not easily adaptable for use as model aggregators. 
Existing model aggregators for crowd text answer aggregation (e.g., \cite{ModelEnsembleSummary, textaggregationdataset}) are mainly extractive aggregation methods and select the potential optimal one from multiple crowd answers. 
Given the instance set $\mathcal{Q}$, worker set $\mathcal{W}$ and answer set $\mathcal{A}$, a model aggregator estimates the true answer $\hat{\mathcal{Z}}$ by selecting one optimal answer $\hat{z}_i$ from $\mathcal{A}_i$ for each instance $q_i$, i.e., the answer aggregation can be defined as $\hat{\mathcal{Z}} = \textnormal{Agg}(\mathcal{Q}, \mathcal{W}, \mathcal{A})$. Note that, in this study, only model aggregators are extractive aggregators. Crowd aggregators and LLM aggregators are abstractive aggregators because they read the raw crowd answers and generate aggregated answers in their own words. 

\subsection{Model Aggregators}
We utilize several aggregation approaches from existing works as the model aggregators. 
These approaches utilize an encoder $e(\cdot)$ to convert the text into embeddings. 

\noindent
\textbf{Sequence Majority Voting (SMV): } 
It is a na\"ive but typical answer aggregation approach that is adapted from majority voting. 
For each instance, it estimates the embeddings of the true answers by $\hat{e}_i = mean(e(\mathcal{A}_i))$, and selects the worker answer $\hat{z}_i = \arg\max_{a_i^j} sim(e(a_i^j),\hat{e}_i).$ 

\noindent
\textbf{Sequence Maximum Similarity (SMS): } For each instance, SMS \cite{ModelEnsembleSummary} selects the worker answer which has the largest sum of similarity with other answers to this question. It can be regarded as creating a kernel density estimator and selecting the maximum density answer. The kernel function uses the cosine similarity. The formulation is  
$\hat{z}_i = \arg\max_{a_i^{j_1}}\sum_{j_1\neq j_2} sim(e(a_i^{j_1}),e(a_i^{j_2})).$ 

\noindent
\textbf{Reliability Aware Sequence Aggregation (RASA): } 
RASA \cite{textaggregationdataset} models the worker reliability $\theta$ to strengthen the influences of answers provided by the workers with higher estimated reliability. 
It first estimates the embeddings of the true answers considering worker reliability. It  iteratively estimates $\theta$ and $\hat{e}_i$ until convergence, $\theta_j = \frac{{\chi}^2_{(\alpha/2,|\mathcal{A}^j|)}}{\sum_i||e(a_i^j)-\hat{e}_i||^2}, \hat{e}_i = \frac{\sum_j \theta_je(a_i^j) }{\sum_j \theta_j},$ 
where ${\chi}^2$ is the chi-squared distribution and the significance level $\alpha$ is set as 0.05 empirically. $\hat{e}_i$ can be initialized by using the SMV method. 
After that, it selects a worker answer that is most similar to the embeddings of the estimated true answer $\hat{e}_i$. 

SMV and SMS are instance-wise aggregators that utilize the answers of an instance as the input. RASA is a dataset-wise aggregator that leverages the potential relations among workers and instances to estimate the answers for all instances. From this viewpoint, the crowd aggregators and LLM aggregators are instance-wise aggregators. 

